Modeling the Quality of Dialogical Explanations

Explanations are pervasive in our lives. Mostly, they occur in dialogical form where an {\em explainer} discusses a concept or phenomenon of interest with an {\em explainee}. Leaving the explainee with a clear understanding is not straightforward due to the knowledge gap between the two participants. Previous research looked at the interaction of explanation moves, dialogue acts, and topics in successful dialogues with expert explainers. However, daily-life explanations often fail, raising the question of what makes a dialogue successful. In this work, we study explanation dialogues in terms of the interactions between the explainer and explainee and how they correlate with the quality of explanations in terms of a successful understanding on the explainee's side. In particular, we first construct a corpus of 399 dialogues from the Reddit forum {\em Explain Like I am Five} and annotate it for interaction flows and explanation quality. We then analyze the interaction flows, comparing them to those appearing in expert dialogues. Finally, we encode the interaction flows using two language models that can handle long inputs, and we provide empirical evidence for the effectiveness boost gained through the encoding in predicting the success of explanation dialogues.

==> table-dlg-act-dist.tex <==
\begin{table}[t]%
	\centering
	\small
	\setlength{\tabcolsep}{3.0pt}%
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{lrrrrr}
		\toprule
		& \multicolumn{5}{c}{\bf Score Distribution} \\
		\cmidrule(lr){2-6}
		{\bf Dialogue Acts} &  1 & 2 & 3 & 4 & 5 \\
		\midrule
			(D09) Info. Statement & 19\% & 12\% & 23\% & 18\% & \bf 28\% \\
			(D03) Question & 580 &  13\% & 23\% & 15\% & 25\%  \\
			(D08) Disagreement &  \bf 59\% & 14\% & 18\% & 6\% & 2\%  \\
			(D02) What/how Ques. & \bf 30\% & 17\% & 20\% & 15\% & 18\% \\
			(D06) Answer & 31\% & 18\% & 11\% & 18\% & 22\%  \\
			(D07) Agreement & 17\% & 7\% & 18\% & \bf 22\% & \bf 35\%  \\
			(D01) Check Question &  32\% & 18\% & 21\% & 14\% & 15\%  \\
			(D05) Disconfirm. &  \bf 39\% & 16\% & 25\% & 11\% & 10\%  \\
			(D04) Confirm. &  28\% & 13\% & 16\% & 17\% & 25\%  \\
			(D10) Other &  37\% & 13\% & 15\% & 15\% & 19\% \\
		\bottomrule
	\end{tabular}
	\caption{The frequency of dialogue acts in our dataset broken  into each of the explanation quality levels [1-5]. Highlighted in bold values that distinguish the presence of these moves in high quality dialogues compared to low quality ones.}
	\label{table-exp-move-flows}
\end{table}


==> table-exp-move-dist.tex <==
\begin{table}[t]%
	\centering
	\small
	\setlength{\tabcolsep}{2.0pt}%
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{lrrrrrr}
		\toprule
		& & \multicolumn{5}{c}{\bf Score Distribution} \\
		\cmidrule(lr){3-7}
		{\bf Explanation Moves} & Freq. & 1 & 2 & 3 & 4 & 5 \\
		\midrule
			(E03) Provide Exp. & 1256 & 22\% & 15\% & 25\% & 17\% & 21\% \\
			(E04) Ask Exp. & 1040 & 25\% & 15\% & 22\% & 15\% & 23\% \\
			(E07) Prov. Feedback & 924 & \bf 40\% & 11\% & 13\% & 14\% & 22\% \\
			(E06) Sig. Non-Under. & 108 & \bf 53\% & 14\% & 14\% & 12\% & 7\% \\
			(E05) Sig. Under. & 45 & 20\% & 13\% & 22\% & 13\% & \bf 31\% \\
			(E08) Provide Assess. & 18 & \bf 72\% & 0\% & 22\% & 6\% & 0\% \\
			(E02) Test prior know. & 17 & \bf 59\% & 18\% & 18\% & 0\% & 6\%  \\
			(E01) Test Underst. & 17 & \bf 53\% & 24\% & 6\% & 12\% & 6\% \\
			(E10) Other & 16 & 31\% & 19\% & 31\% & 19\% & 0\% \\
			(E09) Extra. Info. & 16 & \bf 62\% & 25\% & 6\% & 0\% & 6\% \\
		\bottomrule
	\end{tabular}
	\caption{The frequency of explanation moves in our dataset broken  into each of the explanation quality levels [1-5]. Highlighted in bold values that distinguish the presence of these moves in high quality dialogues compared to low quality ones.}
	\label{table-exp-move-flows}
\end{table}



==> table-quality-automatic-evaluation-on-pred-labels.tex <==
\begin{table}[t]%
	\centering
	\small
	\setlength{\tabcolsep}{1.5pt}%
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{lrr}
		\toprule
		\bf  Approach 	& \bf MAE & \bf MSE \\
		\midrule
		HatFormer-Baseline &1.401 &  1.126 \\
		HatFormer w/ exp-move-encoder &1.388 & 1.083\\
		\addlinespace
		LongFormer-Baseline                         &1.289  & 1.011 \\
		LongFormer w/ exp-move-encoder & \bf 1.253  & \bf 0.969 \\
		\addlinespace
		Average Baseline  & 0.00 &  0.00 \\
		\bottomrule
	\end{tabular}
	\caption{The Mean Absolute Error (MAE) and Mean Squared Error (MSE) for the best variation of our approach when using the predicted labels of explanation moves rather than the ground-truth}
\end{table}



==> table-quality-automatic-evaluation.tex <==
\begin{table}[t]%
	\centering
	\small
	\setlength{\tabcolsep}{1.2pt}%
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{lrrrr}
		\toprule
		& \multicolumn{2}{c}{\bf Ground Truth} & \multicolumn{2}{c}{\bf Preds.} \\
		\cmidrule(lr){2-3} \cmidrule(lr){4-5}
		\bf  Approach 	& \bf RMSE & \bf MAE & \bf RMSE & \bf MAE\\
		\midrule
		Average Baseline  & 1.568 &  1.368 & - &  - \\
		\addlinespace
		HatFormer & 1.481 &  1.293 & - &  - \\
		HatFormer w/ Dlg. Acts & \em 1.439  & \em 1.233 & 1.439 &  1.233 \\
		HatFormer w/ Exp. Moves &1.538 & 1.287 & 1.537 &  1.287 \\
		HatFormer w/ Topics &  1.543  & 1.289 & 1.543 &  1.289 \\
		%HatFormer w/ all-encoder & 1.746  & 1.391 \\
		\addlinespace
		LongFormer                             & 1.364 &  1.048 & - & - \\
		LongFormer w/ Dlg. Acts       & {*}1.215 & {*}0.946 & {*}1.215 &  {*}0.947 \\
		LongFormer w/ Exp. Moves & \bf \em {*}1.192  & \bf \em {*}0.956 & {*}1.192 &  {*}0.956 \\
		LongFormer w/ Topics  & {*}1.223  &  {*}0.956 & {*}1.223 &  {*}0.955 \\
		%LongFormer w/ all-encoder                & 1.412  & 1.062 \\
		\bottomrule
	\end{tabular}
	\caption{The Root Mean Squared Error (RMSE) and Mean Absolute Error (MAE) scores for our approach with different encoders and the corresponding baselines (HatFormer-baseline and LongFormer-baseline) that do not consider the interaction flows, as well as the average baseline}
	\label{table:quality-pred-results}
\end{table}



==> table-topic-func-flows.tex <==
\begin{table*}[t]%
	\centering
	\small
	\setlength{\tabcolsep}{3.5pt}%
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{llrrrrrr}
		\toprule
		&  & & \multicolumn{5}{c}{\bf Score Distribution} \\
		\cmidrule(lr){4-8}
		& {\bf Explanation Move Flow} & Freq. & 1 & 2 & 3 & 4 & 5 \\
		\midrule
		1 & (main, main, main, main, main, main) & 17.6\% & 14.6\% & 15.9\% & 11.0\% & 19.5\% & \bf 39.0\% \\
		2 & (main, main, main, main, main, main, main) & 2.8\% & 38.5\% & 7.7\% & 7.7\% & 38.5\% & 7.7\% \\
		3 & (main, other, other, other, other, other) & 2.6\% & \bf 91.7\% & -- & -- & -- & 8.3\% \\
		4 & (main, other, other, other, other, other, other) & 2.4\% & \bf 63.6\% & 9.1\% & 18.2\% & 9.1\% & -- \\
		5 & (main, sub, sub, sub, sub, sub) & 2.1\% & 10.0\% & 30.0\% & 20.0\% & 20.0\% & 20.0\% \\
		6 & (main, main, main, other, other, other) & 1.5\% & 28.6\% & -- & 14.3\% & 14.3\% & \bf 42.9\% \\
		7 & (main, main, sub, main, main, main) & 1.3\% & -- & 16.7\% & 16.7\% & 50.0\% & 16.7\% \\
		\midrule
		& Overall distribution & 100.0\% & 26.1\% & 13.5\% & 17.3\% & 17.6\% & 25.5\% \\
		\bottomrule
	\end{tabular}
	\caption{The most frequent dialogue act flows in our dataset broken into their frequency in each of the explanation quality levels [1-5]. Highlighted in bold values that distinguish the presence of these flows in high quality dialogues compared to low quality ones.}
	\label{table-topic-func-flows}
\end{table*}


